ERNIE-Search: Bridging Cross-Encoder with Dual-Encoder via Self On-the-fly Distillation for Dense Passage Retrieval

Neural retrievers based on pre-trained language models (PLMs), such as dual-encoders, have achieved promising performance on the task of open-domain question answering (QA). Their effectiveness can further reach new state-of-the-arts by incorporating cross-architecture knowledge distillation. However, most of the existing studies just directly apply conventional distillation methods. They fail to consider the particular situation where the teacher and student have different structures. In this paper, we propose a novel distillation method that significantly advances cross-architecture distillation for dual-encoders. Our method 1) introduces a self on-the-fly distillation method that can effectively distill late interaction (i.e., ColBERT) to vanilla dual-encoder, and 2) incorporates a cascade distillation process to further improve the performance with a cross-encoder teacher. Extensive experiments are conducted to validate that our proposed solution outperforms strong baselines and establish a new state-of-the-art on open-domain QA benchmarks.

==> fig/modeltype.tex <==
\begin{figure*}[tbp]
	\centering
		\includegraphics[width=1.0\textwidth]{./attachments/modeltype.pdf}
		%\captionsetup{width=0.95\textwidth}
	\caption{\textbf{The comparison between Sparse Transformer (ST) and Hierarchical Sparse Transformer (HST)}. \textbf{(a)} Sparse Transformer mainly consists of \colorbox{light_blue}{global attention} and \colorbox{dark_blue}{local attention}.
	\textbf{(b)} The bottleneck that existed in ST: all the sequence information is compressed into a fixed size vector. \textbf{(c)} In HST, \colorbox{green}{representative tokens} are inserted into local attention for hierarchical attention. \textbf{(d)} Information flow demonstration for HST: interaction between representative nodes can increase the path of global information interaction.}
	\label{fig:model_type}
\end{figure*}
